HardScope: Thwarting DOP with Hardware-assisted Run-time Scope Enforcement

Widespread use of memory unsafe programming languages (e.g., C and C++) leaves many systems vulnerable to memory corruption attacks. A variety of defenses have been proposed to mitigate attacks that exploit memory errors to hijack the control flow of the code at run-time, e.g., (fine-grained) randomization or Control Flow Integrity. However, recent work on data-oriented programming (DOP) demonstrated highly expressive (Turing-complete) attacks, even in the presence of these state-of-the-art defenses. Although multiple real-world DOP attacks have been demonstrated, no efficient defenses are yet available. We propose run-time scope enforcement (RSE), a novel approach designed to efficiently mitigate all currently known DOP attacks by enforcing compile-time memory safety constraints (e.g., variable visibility rules) at run-time. We present HardScope, a proof-of-concept implementation of hardware-assisted RSE for the new RISC-V open instruction set architecture. We discuss our systematic empirical evaluation of HardScope which demonstrates that it can mitigate all currently known DOP attacks, and has a real-world performance overhead of 3.2% in embedded benchmarks.

==> sections/07-extensions.tex <==
\section{Extensions}
\label{sec:extensions}








\myparagraph{Deeply nested pointers}
Keeping track of SRS entries is a challenge when deeply nested data structures are delegated, e.g., when the head of a linked list is passed as an argument. Our current PoC Instrumentation Engine
cannot automatically infer the complete set of SRS entries that should be delegated when a callee receives a pointer to beginning of the nested pointer chain. Additionally, the number of SRS entries that must be accumulated and delegated for large nested data structures result in more frequent stalls at run time (cf. additional profiling on CoreMark in Appendix~\ref{appx:coremark_config}).   

To handle delegation of such complex data structures, the \SHORTNAME Instrumentation Engine must infer the relationship between linked data structures and emit instructions to allow \SHORTNAME hardware to derive the complete set of SRS entries that must be delegated for that structure. Wrapper functions for standard data structures can help. Sophisticated program analysis aided by developer annotations may also be used to generate such wrappers automatically. In addition, the \SHORTNAME hardware can be enhanced to use compile-time instrumentation to aggregate related SRS entries to improve the efficiency of nested pointer delegations by storing their entries in dedicated memory.
\ifabridged
\else
Since complex data structures are likely to remain resident in memory over a portion of the program's execution, their entries could be stored in dedicated memory to ease sharing between each execution context requiring access. This would avoid the need of repeatedly copy relevant entries, and aid in keeping the entries for each allowed execution context synchronized as changes are made to the data structure.
\fi


